Simplified Khovanov-Rozansky Chain Complexes of Open 2-braids

Motivated by the works of Krasner [arXiv:0801.4018] and Lobb [arXiv:1103.1412], we simplify the Khovanov-Rozansky chain complexes of open 2-braids. As an application, we show that, for a knot containing a "long" 2-braid, the sl(N) Rasmussen invariant of this knot depends linearly on the length of this 2-braid. We refine this result for (2,2k+1) cable knots and, as a simple corollary, compute the sl(2) Rasmussen invariants of (2,2k+1) cables of slice and amphicheiral knots.

==> MOYII-1.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(40,20)(0,7)

\qbezier(10,10)(10,20)(20,20)

\qbezier(10,10)(10,0)(20,0)

\qbezier(30,10)(30,20)(20,20)

\qbezier(30,10)(30,0)(20,0)

\linethickness{3pt}

\put(0,10){\line(1,0){10}}

\put(30,10){\line(1,0){10}}

\end{picture}

==> MOYII-2.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(40,20)(0,7)


\linethickness{3pt}

\put(0,10){\line(1,0){40}}

\end{picture}

==> fork-21.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(70,40)(10,-10)

\qbezier(50,10)(50,20)(62,20)

\qbezier(50,10)(50,0)(62,0)

\put(80,20){\vector(-1,0){12}}

\put(80,0){\vector(-1,0){12}}

\put(65,-10){\line(0,1){40}}

\linethickness{3pt}

\put(10,10){\line(1,0){40}}

\end{picture}

==> fork-22.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(70,40)(10,-10)

\qbezier(50,10)(50,20)(62,20)

\qbezier(50,10)(50,0)(62,0)

\put(80,20){\vector(-1,0){18}}

\put(80,0){\vector(-1,0){18}}

\put(30,-10){\line(0,1){40}}

\linethickness{3pt}

\put(10,10){\line(1,0){16}}

\put(34,10){\line(1,0){16}}

\end{picture}

==> fork-41.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(70,40)(10,-10)

\qbezier(50,10)(50,20)(62,20)

\qbezier(50,10)(50,0)(62,0)

\put(80,20){\vector(-1,0){12}}

\put(80,0){\vector(-1,0){12}}

\put(65,-10){\line(0,1){40}}

\linethickness{3pt}

\put(65,-10){\line(0,1){40}}

\put(10,10){\line(1,0){40}}

\end{picture}

==> lemma-basis.tex <==
\begin{figure}[ht]
\[
\xymatrix{
\widetilde{\Gamma}: & \input{wide-edge-long-split-closed} &&& \widetilde{\Gamma}': &   \input{wide-edge-long-closed}
}
\]

\caption{}\label{basis-MOY-decomp-II-fig}

\end{figure}


\begin{lemma}\label{lemma-basis-MOY-decmop-II}
Let $\widetilde{\Gamma}$ and $\widetilde{\Gamma}'$ be the closed MOY graph in Figure \ref{basis-MOY-decomp-II-fig}. Then $H(\widetilde{\Gamma}')$ is a free module over the base ring with the basis 
\begin{equation}\label{basis-gamma-prime}
\{x_1^i x_2^j ~|~ 0\leq i \leq N-1,~ 0 \leq j \leq N-2\}
\end{equation}
and $H(\widetilde{\Gamma})$ is a free module over the base ring with the basis 
\begin{equation}\label{basis-gamma}
\{x_1^i x_2^j x_5^\ve~|~ 0\leq i \leq N-1,~ 0 \leq j \leq N-2,~ \ve=0,1\}.
\end{equation}
\end{lemma}

\begin{proof}
We only prove the lemma for $H_{x^{N+1}-ax}$. The proofs for the other two versions of the Khovanov-Rozansky homology are very similar and left to the reader. To simplify the notations, $C$ and $H$ in this proof means $C_{x^{N+1}-ax}$ and $H_{x^{N+1}-ax}$.

There is a unique way to express the symmetric polynomial $(x^{N+1}-ax) + (y^{N+1}-ay)$ as a polynomial $g(x+y,xy)$. Let 
\begin{eqnarray*}
u_{ijkl} & = & u(x_i,x_j,x_k,x_l) =
\frac{g(x_i+x_j,x_ix_j)-g(x_k+x_l,x_ix_j)}{x_i+x_j-x_k-x_l}, \\
v_{ijkl} & = & v(x_i,x_j,x_k,x_l) =
\frac{g(x_k+x_l,x_ix_j)-g(x_k+x_l,x_kx_l)}{x_ix_j-x_kx_l}.
\end{eqnarray*}
These are polynomials in $x_i,x_j,x_k,x_l$. By definition,
\[
C(\widetilde{\Gamma}') = \left(%
\begin{array}{cc}
  u_{1212} & 0 \\
  v_{1212} & 0 
\end{array}%
\right)_{\C[a,x_1,x_2]}\{-1\}.
\]
By \cite[Lemma 4.1]{Wu-color}, we have
\begin{eqnarray*}
u_{1212} &=& a+ (N+1) \sum_{i=0}^{N}x_1^i x_2^{N-i}, \\
v_{1212} &=& -(N+1)  \sum_{i=0}^{N-1}x_1^i x_2^{N-i-1}.
\end{eqnarray*}
From \cite[Lemma 2.4]{Wu-color-equi}, we know
\[
H(\widetilde{\Gamma}') \cong \left(\sfrac{\C[a,x_1,x_2]}{(u_{1212},v_{1212})}\right) \{q^{3-2N}\}.
\]
It is simple algebra to verify that $\left(\sfrac{\C[a,x_1,x_2]}{(u_{1212},v_{1212})}\right)$ is a free $\C[a]$-module with basis \eqref{basis-gamma-prime}.

From the proof of the second MOY decomposition in \cite[Proposition 30]{KR1}, we see that there is a decomposition
\[
C(\widetilde{\Gamma}) \simeq C(\widetilde{\Gamma}')\{q^{-1}\} \oplus (x_5 \cdot C(\widetilde{\Gamma}'))\{q^{-1}\}.
\]
So basis \eqref{basis-gamma-prime} of $H(\widetilde{\Gamma}')$ leads to basis \eqref{basis-gamma} of $H(\widetilde{\Gamma})$
\end{proof}



$\mathbb{m}$

